DecompOpt: Controllable and Decomposed Diffusion Models for Structure-based Molecular Optimization

Recently, 3D generative models have shown promising performances in structure-based drug design by learning to generate ligands given target binding sites. However, only modeling the target-ligand distribution can hardly fulfill one of the main goals in drug discovery -- designing novel ligands with desired properties, e.g., high binding affinity, easily synthesizable, etc. This challenge becomes particularly pronounced when the target-ligand pairs used for training do not align with these desired properties. Moreover, most existing methods aim at solving \textit{de novo} design task, while many generative scenarios requiring flexible controllability, such as R-group optimization and scaffold hopping, have received little attention. In this work, we propose DecompOpt, a structure-based molecular optimization method based on a controllable and decomposed diffusion model. DecompOpt presents a new generation paradigm which combines optimization with conditional diffusion models to achieve desired properties while adhering to the molecular grammar. Additionally, DecompOpt offers a unified framework covering both \textit{de novo} design and controllable generation. To achieve so, ligands are decomposed into substructures which allows fine-grained control and local optimization. Experiments show that DecompOpt can efficiently generate molecules with improved properties than strong de novo baselines, and demonstrate great potential in controllable generation tasks.

==> tables/decomp_benefits.tex <==
\begin{table*}[ht]
    \vspace{-0.05in}
    \small
    \centering
    \caption{TODO}
    \vspace{-0.07in}
    % \begin{adjustbox}{width=1\textwidth}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{c|cc}
    \toprule
    % \diagbox{Model}{Metric} 
    \multirow{2}{*}{Method} 
    & \multicolumn{2}{c}{Vina Min ($\downarrow$)} \\
    & Avg. & Med. \\ 
    \midrule
    DecompDiff & -6.01 & -5.98 \\
    Molecule-level Opt. & -6.62 & -6.66 \\
    Arm-level Opt. & -6.72 & -6.72 \\
    \bottomrule
    \end{tabular}\label{tab:mol_wise_table}
    \renewcommand{\arraystretch}{1}
    % \end{adjustbox}
    \vspace{-0.1in}
\end{table*}

==> tables/single_obj_opt.tex <==
\definecolor{darkgreen}{RGB}{34,139,34}

\begin{wraptable}{r}{0.6\textwidth}
%\begin{table*}[htbp]
    \fontsize{8}{9.5}\selectfont
    \centering
    \resizebox{0.6\textwidth}{!}{%
    \caption{Summary of results of single-objective optimization. The improvements of \method over the baseline are highlighted in \textcolor{darkgreen}{green}.}
    %\vspace{-0.07in}
    % \begin{adjustbox}{width=1\textwidth}
    \renewcommand{\arraystretch}{1.3}
    \begin{tabularx}{0.6\textwidth}{c|cc|cc}
    \toprule
    % \diagbox{Model}{Metric} 
    \multirow{2}{*}{Optimized\\}
    & \multicolumn{2}{c|}{DecompDiff} & \multicolumn{2}{c}{\method} \\
    Property & Avg. & Med. & Avg. & Med. \\ 
    \midrule
    QED ($\uparrow$) & 0.48 & 0.48 & 0.52 \textcolor{darkgreen}{(+8.3\%)} & 0.53 \textcolor{darkgreen}{(+10.4\%)} \\
    SA ($\uparrow$) & 0.67 & 0.66 & 0.74 \textcolor{darkgreen}{(+10.5\%)} & 0.74 \textcolor{darkgreen}{(+12.1\%)} \\
    Vina Min ($\downarrow$) & -6.01 & -5.98 & -6.72 \textcolor{darkgreen}{(+11.8\%)} & -6.72 \textcolor{darkgreen}{(+12.4\%)} \\
    \bottomrule
    \end{tabularx} %
    }
    \label{tab:single_objective_table}
    \renewcommand{\arraystretch}{1}
    % \end{adjustbox}
    \vspace{-0.1in}
%\end{table*}
\end{wraptable}


\definecolor{darkgreen}{RGB}{34,139,34}

==> wrap_figs/diversity.tex <==
\begin{wrapfigure}{r}{0.46\textwidth}
\centering
    \vspace{-0.16in}
    % \includegraphics[trim={4cm 0 4cm 0.5cm},clip,width=0.62\textwidth]
    \includegraphics[width=0.46\textwidth]{figures/diversity_succ_rate_scatter.pdf}
    \captionof{figure}{Trade-off of Success Rate and diversity. Each point with coordinate $(x,y)$ represents a pocket with Success Rate $x$ and diversity $y$. The closer to the top right, the better. }
    \vspace{-0.4in}
    \label{fig:diversity_scatter}
\end{wrapfigure}

==> wrap_figs/r-group.tex <==
\begin{wrapfigure}{r}{0.58\textwidth}
\centering
    % \vspace{-0.16in}
    % \includegraphics[trim={4cm 0 4cm 0.5cm},clip,width=0.62\textwidth]
    \includegraphics[width=0.58\textwidth]{figures/r-group-viz.pdf}
    \captionof{figure}{Visualization of reference binding molecules (left column), molecules generated by \method (middle and right column) with 30 rounds of optimization on protein 3DAF (top row) and 4F1M (bottom row). Optimized R-group are highlighted in red.}
    \label{fig:R-group}
    % \vspace{-0.16in}
\end{wrapfigure} 

==> wrap_figs/scaffold_hopping.tex <==
\begin{wrapfigure}{r}{0.58\textwidth}
\centering
    % \vspace{-0.16in}
    % \includegraphics[trim={4cm 0 4cm 0.5cm},clip,width=0.62\textwidth]
    \includegraphics[width=0.58\textwidth]{figures/scaffold_hopping_final.pdf}
    \captionof{figure}{Examples of scaffold hopping accomplished by \method. For each row, the left image shows the reference ligand, the middle and right images are two examples generated by \method. Reference and generated scaffolds are highlighted in green.}
    \label{fig:scaffold_hopping}
    \vspace{-0.4in}
\end{wrapfigure}
